Learning Causal Dynamics Models in Object-Oriented Environments

Causal dynamics models (CDMs) have demonstrated significant potential in addressing various challenges in reinforcement learning. To learn CDMs, recent studies have performed causal discovery to capture the causal dependencies among environmental variables. However, the learning of CDMs is still confined to small-scale environments due to computational complexity and sample efficiency constraints. This paper aims to extend CDMs to large-scale object-oriented environments, which consist of a multitude of objects classified into different categories. We introduce the Object-Oriented CDM (OOCDM) that shares causalities and parameters among objects belonging to the same class. Furthermore, we propose a learning method for OOCDM that enables it to adapt to a varying number of objects. Experiments on large-scale tasks indicate that OOCDM outperforms existing CDMs in terms of causal discovery, prediction accuracy, generalization, and computational efficiency.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> related_works.tex <==
\subsection{Object-oriented reinforcement learning}

Several studies investigate combing RL with the object-oriented framework, which is natural to describe environments and brings copious opportunity for generalization. Early studies includes Relational RL \cite{goos_relational_1998} and Object-oriented RL \cite{diuk_object-oriented_2008}, which use similar variants of MDP to describe environments through classes, objects, and the attributes of objects. Following their work, \citet{zambaldi_relational_2018} proposed an approach to learn interpretable policies by extracting the relation between objects. Only a few studies investigate object-oriented dynamics models, such like Object-Oriented Dynamics Predictor (OODP) \cite{zhu_object-oriented_2018,zhu_object-oriented_2019}, which predicts the movement of objects in a 2-dimensional image. To the best of our knowledge, our OOC-model is the first object-oriented dynamics model that accepts arbitrary definition of classes.

\subsection{Causal reinforcement learning}

Recently, integrating RL with causality has attracted much interest from researchers. Studies of causal RL (CRL) can be roughly devided into two categories. The first category cares about \textit{macro causalities}, which exist among macro elements of MDPs like states, actions, observations, rewards, and noise. Studies of this kind usually presuppose known CGs shared by a range of environments, and derive new algorithms with improved the robustness, sample efficiency based on thes CGs \cite{buesing_woulda_2018, lu_deconfounding_2018, zhang_invariant_2020, liao_instrumental_2021}. In contrast, the second category focuses on \textit{micro causalities}, which exists among specific components of the environment (e.g., components $s_i$ of the state vector $\bm{s}$). These micro causalities are usually distinctive in each environment. Therefore, studies of this kind usually require expert knowledge or use causal discovery to obtain the CGs. Micro causalities can benefit RL in many ways, including 1) improving optimizing hierarchy of tasks \cite{peng_causality-driven_2022}, 2) explaining agents' decisions \cite{madumal_explainable_2020, madumal_distal_2020}, 3) improving generalization of policies \cite{nair_causal_2019}, and 4) improving generalization of dynamics models through CDMs \cite{ding_generalizing_2022, wang_causal_2022, zhu_offline_2022}. To the best of our knowledge, our OOC-model is the first model to combine causality with object-oriented framework in RL.
